Intensity Harmonization for Airborne LiDAR

Constructing a point cloud for a large geographic region, such as a state or country, can require multiple years of effort. Often several vendors will be used to acquire LiDAR data, and a single region may be captured by multiple LiDAR scans. A key challenge is maintaining consistency between these scans, which includes point density, number of returns, and intensity. Intensity in particular can be very different between scans, even in areas that are overlapping. Harmonizing the intensity between scans to remove these discrepancies is expensive and time consuming. In this paper, we propose a novel method for point cloud harmonization based on deep neural networks. We evaluate our method quantitatively and qualitatively using a high quality real world LiDAR dataset. We compare our method to several baselines, including standard interpolation methods as well as histogram matching. We show that our method performs as well as the best baseline in areas with similar intensity distributions, and outperforms all baselines in areas with different intensity distributions. Source code is available at https://github.com/mvrl/lidar-harmonization .

==> old_unused/4method.tex <==
% \section{Method}

% In this section, we describe the three methods for harmonization. We introduce a naive baseline interpolation method which we then improve by leveraging the PointNet architecture. These methods are finally compared to histogram matching, which serves as the primary baseline for our method. 

% \subsection{Interpolation}

% Given a target scan $P_t$ and a source scan $P_s$, we can interpolate the intensity value of $P_s$ at every point from $P_t$ where $P_t$ overlaps with $P_s$. These interpolated values form pairs with the target point's intensity from $P_t$. A regression is applied to these pairs to solve for the transformation that harmonizes $P_s$ to $P_t$. Our initial baseline method uses standard linear interpolation methods. The regression is performed by least squares approximation as well as by a multilayer perceptron (MLP). 

% Extending this, a pointnet architecture is used to approximate better interpolations. The pointnet is trained on source neighborhoods taken from the overlap regions between $P_t$ and $P_s$ which are centered around target points from $P_t$.
    
% \textbf{Model Training} We utilize Huber Loss $\rho$ for the interpolated value at every point as well as for the harmonized values within the overlap. The loss for our model is formulated by the following:





% \textbf{Network Optimization} Pytorch is used for model training. Adam is chosen for the optimizer, with Cyclic learning rate (scaling factor of 2), an upper bound of $10^{-3}$ and a lower bound of $10^{-6}$. A batch size of 50 is used during training. Our network architecture can be seen in Figure~\ref{fig:architecture}.

% \subsection{Histogram Matching}

% Histogram matching creates a transformation directly from one histogram to another, such that the distributions are aligned. While the previous methods outlined in this paper utilize the information and geometry of the physical points, histogram matching only examines the distribution of intensities, without the need for correspondence between points.


